Stochastic Gradient Descent Meets Distribution Regression

Stochastic gradient descent (SGD) provides a simple and efficient way to solve a broad range of machine learning problems. Here, we focus on distribution regression (DR), involving two stages of sampling: Firstly, we regress from probability measures to real-valued responses. Secondly, we sample bags from these distributions for utilizing them to solve the overall regression problem. Recently, DR has been tackled by applying kernel ridge regression and the learning properties of this approach are well understood. However, nothing is known about the learning properties of SGD for two stage sampling problems. We fill this gap and provide theoretical guarantees for the performance of SGD for DR. Our bounds are optimal in a mini-max sense under standard assumptions.

==> macros_nicole.tex <==


\RequirePackage{wasysym }
%\RequirePackage[isolatin]{inputenc}
\RequirePackage{comment}
\RequirePackage{graphicx}
\RequirePackage{amsmath}%,amsfonts}
\RequirePackage{color}


\usepackage{colortbl}
\usepackage{xcolor}


\definecolor{blue}{rgb}{0.6, 0.4, 1.0} %{0.0,0.0,0.55}
%\definecolor{blue}{rgb}{0.0,0.0,0.55}
\definecolor{red}{rgb}{0.75,0.0,0.0}
\definecolor{green}{rgb}{0.0,0.5,0.0}
\definecolor{bluebell}{rgb}{0.64, 0.64, 0.82}
\definecolor{amethyst}{rgb}{0.6, 0.4, 0.8}
\definecolor{applegreen}{rgb}{0.55, 0.71, 0.0}
\definecolor{awesome}{rgb}{1.0, 0.13, 0.32}
\definecolor{caribbeangreen}{rgb}{0.0, 0.8, 0.6}
 	
\newcommand{\blue}{\color{blue}}
\newcommand{\green}{\color{green}}
\newcommand{\red}{\color{red}}
 
\newcommand{\magenta}{\color{magenta}}
\newcommand{\notice}[1]{\color{magenta} #1}


%\ifx \skiptheorems \thiscommandisnotdefinedtralala  
                 

\RequirePackage{amsthm}


\newtheorem{theorem}{Theorem}[section]
\newtheorem{definition}[theorem]{Definition}
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{corollary}[theorem]{Corollary}

\newtheorem{assumption}[theorem]{Assumption}
% 
% \theoremstyle{remark}
\newtheorem{question}[theorem]{Question}
\newtheorem{example}[theorem]{Example}
\newtheorem{remark}[theorem]{Remark}



%\newtheorem{theorem}{Theorem}[section]
%\newtheorem{proposition}[theorem]{Proposition}
%\newtheorem{corollary}[theorem]{Corollary}
%\newtheorem{lemma}[theorem]{Lemma}
%\newtheorem{assumption}[theorem]{Assumption}


%\theoremstyle{definition}
%\newtheorem{definition}[theorem]{Definition}
%\newtheorem{property}[theorem]{Property}
%\newtheorem{example}[theorem]{Example}

%\theoremstyle{remark}
%\newtheorem{remark}[theorem]{Remark}

%\else

%\newtheorem{theorem}{Théorème}[section]
%\newtheorem{proposition}[theorem]{Proposition}
%\newtheorem{corollary}[theorem]{Corollaire}
%\newtheorem{lemma}[theorem]{Lemme}
%\theoremstyle{definition}
%\newtheorem{definition}[theorem]{Définition}
%\newtheorem{property}[theorem]{Propriété}
%\newtheorem{example}[theorem]{Example}
%\theoremstyle{remark}
%\newtheorem{remark}[theorem]{Remarque}
%\fi
%\fi

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\floor}[1]{\lfloor #1 \rfloor}


\DeclareMathOperator{\supp}{supp}

\newcommand{\no}{\nonumber}

% Fonts

\newcommand{\mtc}{\mathcal}
\newcommand{\mbf}{\mathbf}

% Some black magic to remove annoying extra spaces before/after \left* and \right*

\let\originalleft\left
\let\originalright\right
\renewcommand{\left}{\mathopen{}\mathclose\bgroup\originalleft}
\renewcommand{\right}{\aftergroup\egroup\originalright}


% Accents tildes over/underline etc

\newcommand{\wt}[1]{{\widetilde{#1}}}
\newcommand{\wh}[1]{{\widehat{#1}}}
\newcommand{\ol}[1]{\overline{#1}}
\newcommand{\ul}[1]{\underline{#1}}



\RequirePackage{xstring}

\newcommand{\ind}[1]{{\mbf{1}\{#1\}}}
\newcommand{\paren}[2][a]{%
\IfEqCase{#1}{%
{a}{\left(#2\right)}%
{0}{(#2)}%
{1}{\big(#2\big)}%
{2}{\Big(#2\Big)}%
{3}{\bigg(#2\bigg)}%
{4}{\Bigg(#2\Bigg)}%
}[\PackageError{paren}{Undefined option to paren: #1}{}]%
}
\newcommand{\norm}[2][a]{%
\IfEqCase{#1}{%
{a}{\left\lVert#2\right\rVert}%
{0}{\lVert#2\rVert}%
{1}{\big\lVert#2\big\rVert}%
{2}{\Big\lVert#2\Big\rVert}%
{3}{\bigg\lVert#2\bigg\rVert}%
{4}{\Bigg\lVert#2\Bigg\rVert}%
}[\PackageError{norm}{Undefined option to norm: #1}{}]%
}
\newcommand{\brac}[2][a]{%
\IfEqCase{#1}{%
{a}{\left[#2\right]}%
{0}{[#2]}%
{1}{\big[#2\big]}%
{2}{\Big[#2\Big]}%
{3}{\bigg[#2\bigg]}%
{4}{\Bigg[#2\Bigg]}%
}[\PackageError{brac}{Undefined option to brac: #1}{}]%
}
\newcommand{\inner}[2][a]{%
\IfEqCase{#1}{%
{a}{\left\langle#2\right\rangle}%
{0}{\langle#2\rangle}%
{1}{\big\langle#2\big\rangle}%
{2}{\Big\langle#2\Big\rangle}%
{3}{\bigg\langle#2\bigg\rangle}%
{4}{\Bigg\langle#2\Bigg\rangle}%
}[\PackageError{inner}{Undefined option to inner: #1}{}]%
}
\newcommand{\abs}[2][a]{
\IfEqCase{#1}{%
{a}{\left\vert#2\right\rvert}%
{0}{\vert#2\rvert}%
{1}{\big\vert#2\big\rvert}%
{2}{\Big\vert#2\Big\rvert}%
{3}{\bigg\vert#2\bigg\rvert}%
{4}{\Bigg\vert#2\Bigg\rvert}%
}[\PackageError{inner}{Undefined option to abs: #1}{}]%
}



%\newcommand{\set}[1]{\left\{#1\right\}}


% Autres

\newcommand{\np}{_{_-}}
\newcommand{\pp}{_{_+}}
\newcommand{\defeq}{\stackrel{\cdot}{=}} % this is for
                                % definition-equal, not for number 2
                                % [This comment is (c) Gabór L. ]
\newcommand{\bydef}{:=}       % an alternative to defeq

% Operateurs proba

%\newcommand{\var}[2][a]{{\rm Var}\brac[#1]{#2}}
\newcommand{\cov}[2][a]{{\rm Cov}\brac[#1]{#2}} 
%\newcommand{\e}[2][a]{\mbe\brac[#1]{#2}}
\newcommand{\ee}[3][a]{\mbe_{#2}\brac[#1]{#3}}
\newcommand{\prob}[2][a]{\mbp\brac[#1]{#2}}
\newcommand{\probb}[3][a]{\mbp_{#2}\brac[#1]{#3}}


% Operateurs

\def\argmin{\mathop{\rm Arg\,Min}\limits}
\def\argmax{\mathop{\rm Arg\,Max}\limits}
\def\sgn{\mathop{\rm Sgn}\limits}
\def\tr{\mathop{\rm Tr}\limits}


% abbrev lettres grecques

\newcommand{\al}{\alpha}
\newcommand{\lam}{\lambda}
%\newcommand{\om}{\omega}
%\newcommand{\eps}{\varepsilon}

% abbrev lettres mathcal

\def\cA{{\mtc{A}}}
\def\cB{{\mtc{B}}}
\def\cC{{\mtc{C}}}
\def\cD{{\mtc{D}}}
\def\cE{{\mtc{E}}}
\def\cF{{\mtc{F}}}
\def\cG{{\mtc{G}}}
\def\cH{{\mtc{H}}}
\def\cI{{\mtc{I}}}
\def\cK{{\mtc{K}}}
\def\cL{{\mtc{L}}}
\def\cM{{\mtc{M}}}
\def\cN{{\mtc{N}}}
\def\cO{{\mtc{O}}}
\def\cP{{\mtc{P}}}
\def\cQ{{\mtc{Q}}}
\def\cR{{\mtc{R}}}
\def\cS{{\mtc{S}}}
\def\cT{{\mtc{T}}}
\def\cU{{\mtc{U}}}
\def\cV{{\mtc{V}}}
\def\cW{\mathcal{W}}
\def\cX{\mathcal{X}}
\def\cY{\mathcal{Y}}
\def\cZ{\mathcal{Z}}

% abbrev lettres mathbb

\newcommand{\mbe}{\mathbb{E}}
\newcommand{\mbr}{\mathbb{R}}
\newcommand{\mbp}{\mathbb{P}}
\newcommand{\mbq}{\mathbb{Q}}
\newcommand{\mbi}{\mathbb{I}}
\newcommand{\mbn}{\mathbb{N}}
\newcommand{\mbz}{\mathbb{Z}}
\newcommand{\mbs}{\mathbb{S}}
\newcommand{\mbk}{\mathbb{K}}
\newcommand{\mbg}{\mathbb{G}}
\newcommand{\mbv}{\mathbb{V}}


% abbrev lettres en gras

\newcommand{\bA}{{\mbf{A}}}
\newcommand{\bB}{{\mbf{B}}}
\newcommand{\bD}{{\mbf{D}}}
\newcommand{\bG}{{\mbf{G}}}
\newcommand{\bI}{{\mbf{I}}}
\newcommand{\bJ}{{\mbf{J}}}
\newcommand{\bW}{{\mbf{W}}}
\newcommand{\bX}{{\mbf{X}}}
\newcommand{\bY}{{\mbf{Y}}}
\newcommand{\bZ}{{\mbf{Z}}}


\newcommand{\bp}{{\mbf{p}}}
\newcommand{\boldf}{{\mbf{f}}}
\newcommand{\bx}{{\mbf{x}}}
\newcommand{\by}{{\mbf{y}}}
\newcommand{\bz}{{\mbf{z}}}
\newcommand{\bw}{{\mbf{w}}}
\newcommand{\bv}{{\mbf{v}}}
\newcommand{\barx}{{\bar{x}}}

% frak

\newcommand{\fP}{{\mathfrak{P}}}
\newcommand{\fK}{{\mathfrak{K}}}

\newcommand{\la}{\langle}
\newcommand{\ra}{\rangle}

%\newcommand{\red}[1]{\textcolor{red}{#1}}


\newcommand{\nux}{\nu}


% TODO command

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% A command to put notes in a draft

\newcounter{nbdrafts}
\setcounter{nbdrafts}{0}
\makeatletter
\newcommand{\checknbdrafts}{
\ifnum \thenbdrafts > 0
\@latex@warning@no@line{**********************************************************************}
\@latex@warning@no@line{* The document contains \thenbdrafts \space draft note(s)}
\@latex@warning@no@line{**********************************************************************}
\fi}
\newcommand{\todo}[1]{\addtocounter{nbdrafts}{1}{\color{awesome} #1}}
\makeatother

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcounter{nbnotes}
\setcounter{nbnotes}{0}
\makeatletter
\newcommand{\checknbnotes}{
\ifnum \thenbnotes > 0
\@latex@warning@no@line{**********************************************************************}
\@latex@warning@no@line{* The document contains \thenbnotes \space color note(s)}
\@latex@warning@no@line{**********************************************************************}
\fi}
\newcommand{\note}[1]{\addtocounter{nbnotes}{1}{\color{blue} #1}}%amethyst
\makeatother

